Locomotion and Obstacle Avoidance of a Worm-like Soft Robot

This paper presents a soft earthworm robot that is capable of both efficient locomotion and obstacle avoidance. The robot is designed to replicate the unique locomotion mechanisms of earthworms, which enable them to move through narrow and complex environments with ease. The robot consists of multiple segments, each with its own set of actuators, that are connected through rigid plastic joints, allowing for increased adaptability and flexibility in navigating different environments. The robot utilizes proprioceptive sensing and control algorithms to detect and avoid obstacles in real-time while maintaining efficient locomotion. The robot uses a pneumatic actuation system to mimic the circumnutation behavior exhibited by plant roots in order to navigate through complex environments. The results demonstrate the capabilities of the robot for navigating through cluttered environments, making this development significant for various fields of robotics, including search and rescue, environmental monitoring, and medical procedures.

==> bibtex.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{application}
\BIBentryALTinterwordspacing
B.~Zhang, Y.~Fan, P.~Yang, T.~Cao, and H.~Liao, ``Worm-like soft robot for
  complicated tubular environments,'' \emph{Soft Robotics}, vol.~6, no.~3, pp.
  399--413, 2019, pMID: 31180823. [Online]. Available:
  \url{https://doi.org/10.1089/soro.2018.0088}
\BIBentrySTDinterwordspacing

\bibitem{trueman_1975}
E.~R. Trueman, \emph{The locomotion of soft-bodied animals}.\hskip 1em plus
  0.5em minus 0.4em\relax Edward Arnold, 1975.

\bibitem{Noorani}
M.-R.~S. Noorani, A.~Ghanbari, and S.~Aghli, ``Design and fabrication of a worm
  robot prototype,'' in \emph{2015 3rd RSI International Conference on Robotics
  and Mechatronics (ICROM)}, 2015, pp. 073--078.

\bibitem{Niu}
\BIBentryALTinterwordspacing
H.~Niu, R.~Feng, Y.~Xie, B.~Jiang, Y.~Sheng, Y.~Yu, H.~Baoyin, and X.~Zeng,
  ``Magworm: A biomimetic magnet embedded worm-like soft robot,'' \emph{Soft
  Robotics}, vol.~8, no.~5, pp. 507--518, 2021, pMID: 32822273. [Online].
  Available: \url{https://doi.org/10.1089/soro.2019.0167}
\BIBentrySTDinterwordspacing

\bibitem{kal}
\BIBentryALTinterwordspacing
M.~Sivaperuman~Kalairaj, C.~J. Cai, P.~S, and H.~Ren, ``Untethered origami worm
  robot with diverse multi-leg attachments and responsive motions under
  magnetic actuation,'' \emph{Robotics}, vol.~10, no.~4, p. 118, Nov 2021.
  [Online]. Available: \url{http://dx.doi.org/10.3390/robotics10040118}
\BIBentrySTDinterwordspacing

\bibitem{Yas}
B.~Liu, Y.~Ozkan-Aydin, D.~I. Goldman, and F.~L. Hammond, ``Kirigami skin
  improves soft earthworm robot anchoring and locomotion under cohesive soil,''
  in \emph{2019 2nd IEEE International Conference on Soft Robotics (RoboSoft)},
  2019, pp. 828--833.

\bibitem{Xu}
\BIBentryALTinterwordspacing
L.~Xu, R.~J. Wagner, S.~Liu, Q.~He, T.~Li, W.~Pan, Y.~Feng, H.~Feng, Q.~Meng,
  X.~Zou, Y.~Fu, X.~Shi, D.~Zhao, J.~Ding, and F.~J. Vernerey, ``Locomotion of
  an untethered, worm-inspired soft robot driven by a shape-memory alloy
  skeleton,'' \emph{Scientific Reports}, vol.~12, no.~1, p. 12392, Jul 2022.
  [Online]. Available: \url{https://doi.org/10.1038/s41598-022-16087-5}
\BIBentrySTDinterwordspacing

\bibitem{Du}
\BIBentryALTinterwordspacing
T.~Du, L.~Sun, and J.~Wan, ``A worm-like crawling soft robot with pneumatic
  actuators based on selective laser sintering of tpu powder,''
  \emph{Biomimetics}, vol.~7, no.~4, p. 205, Nov 2022. [Online]. Available:
  \url{http://dx.doi.org/10.3390/biomimetics7040205}
\BIBentrySTDinterwordspacing

\bibitem{Das2023}
\BIBentryALTinterwordspacing
R.~Das, S.~P.~M. Babu, F.~Visentin, S.~Palagi, and B.~Mazzolai, ``An
  earthworm-like modular soft robot for locomotion in multi-terrain
  environments,'' \emph{Scientific Reports}, vol.~13, no.~1, p. 1571, Jan 2023.
  [Online]. Available: \url{https://doi.org/10.1038/s41598-023-28873-w}
\BIBentrySTDinterwordspacing

\bibitem{Wang1}
\BIBentryALTinterwordspacing
Y.~Wang, Z.~Liu, A.~Kandhari, and K.~A. Daltorio, ``Obstacle avoidance path
  planning for worm-like robot using bézier curve,'' \emph{Biomimetics},
  vol.~6, no.~4, p.~57, Sep 2021. [Online]. Available:
  \url{http://dx.doi.org/10.3390/biomimetics6040057}
\BIBentrySTDinterwordspacing

\bibitem{Wang2}
\BIBentryALTinterwordspacing
Y.~Wang, P.~Pandit, A.~Kandhari, Z.~Liu, and K.~A. Daltorio, ``Rapidly
  exploring random tree algorithm-based path planning for worm-like robot,''
  \emph{Biomimetics}, vol.~5, no.~2, p.~26, Jun 2020. [Online]. Available:
  \url{http://dx.doi.org/10.3390/biomimetics5020026}
\BIBentrySTDinterwordspacing

\bibitem{Kandhari}
\BIBentryALTinterwordspacing
A.~Kandhari, Y.~Wang, H.~J. Chiel, and K.~A. Daltorio, ``Turning in worm-like
  robots: The geometry of slip elimination suggests nonperiodic waves,''
  \emph{Soft Robotics}, vol.~6, no.~4, pp. 560--577, 2019, pMID: 31066633.
  [Online]. Available: \url{https://doi.org/10.1089/soro.2018.0080}
\BIBentrySTDinterwordspacing

\bibitem{Gough}
E.~Gough, A.~T. Conn, and J.~Rossiter, ``Planning for a tight squeeze:
  Navigation of morphing soft robots in congested environments,'' \emph{IEEE
  Robotics and Automation Letters}, vol.~6, no.~3, pp. 4752--4757, 2021.

\bibitem{Verma}
D.~Verma, P.~Saxena, and R.~Tiwari, ``Robot navigation and target capturing
  using nature-inspired approaches in a dynamic environment,'' in \emph{2020
  10th International Conference on Cloud Computing, Data Science \& Engineering
  (Confluence)}, 2020, pp. 629--636.

\bibitem{Zhang}
\BIBentryALTinterwordspacing
Q.~Zhang, H.~Fang, and J.~Xu, ``Yoshimura-origami based earthworm-like robot
  with 3-dimensional locomotion capability,'' \emph{Frontiers in Robotics and
  AI}, vol.~8, 2021. [Online]. Available:
  \url{https://www.frontiersin.org/articles/10.3389/frobt.2021.738214}
\BIBentrySTDinterwordspacing

\bibitem{roots}
\BIBentryALTinterwordspacing
I.~Taylor, K.~Lehner, E.~McCaskey, N.~Nirmal, Y.~Ozkan-Aydin, M.~Murray-Cooper,
  R.~Jain, E.~W. Hawkes, P.~C. Ronald, D.~I. Goldman, and P.~N. Benfey,
  ``Mechanism and function of root circumnutation,'' \emph{Proceedings of the
  National Academy of Sciences}, vol. 118, no.~8, p. e2018940118, 2021.
  [Online]. Available:
  \url{https://www.pnas.org/doi/abs/10.1073/pnas.2018940118}
\BIBentrySTDinterwordspacing

\bibitem{Perastaltic}
H.~Omori, T.~Hayakawa, and T.~Nakamura, ``Locomotion and turning patterns of a
  peristaltic crawling earthworm robot composed of flexible units,'' in
  \emph{2008 IEEE/RSJ International Conference on Intelligent Robots and
  Systems}, 2008, pp. 1630--1635.

\end{thebibliography}
